Large-scale geometry of Borel graphs of polynomial growth

We study graphs of polynomial growth from the perspective of asymptotic geometry and descriptive set theory. The starting point of our investigation is a theorem of Krauthgamer and Lee who showed that every connected graph of polynomial growth admits an injective contraction mapping to $(\mathbb Z^n, \|\cdot\|_\infty)$ for some $n\in\mathbb N$. We strengthen and generalize this result in a number of ways. In particular, answering a question of Papasoglu, we construct coarse embeddings from graphs of polynomial growth to $\mathbb Z^n$. Moreover, we only require $n$ to be linear in the asymptotic polynomial growth rate of the graph; this confirms a conjecture of Levin and Linial, London, and Rabinovich "in the asymptotic sense." (The exact form of the conjecture was refuted by Krauthgamer and Lee.) All our results are proved for Borel graphs, which allows us to settle a number of problems in descriptive combinatorics. Roughly, we prove that graphs generated by free Borel actions of $\mathbb Z^n$ are universal for the class of Borel graphs of polynomial growth. This provides a general method for extending results about $\mathbb Z^n$-actions to all Borel graphs of polynomial growth. For example, an immediate consequence of our main result is that all Borel graphs of polynomial growth are hyperfinite, which answers a well-known question in the area. As another illustration, we show that Borel graphs of polynomial growth support a certain combinatorial structure called toast. An important technical tool in our arguments is the notion of padded decomposition from computer science, which is closely related to the concept of asymptotic dimension due to Gromov. Along the way we find an alternative, probabilistic proof of a theorem of Papasoglu that graphs of asymptotic polynomial growth rate $\rho<\infty$ have asymptotic dimension at most $\rho$ and establish the same bound in the Borel setting.

==> abstract.tex <==
 Let $\mathsf{Grid}_{n, \infty}$ be the $n$-dimensional grid graph with diagonals, i.e., the graph with vertex set $\mathbb{Z}^n$ in which two vertices $u$, $v \in \mathbb{Z}^n$ are adjacent if and only if $\|u - v\|_\infty = 1$. In 1995, Levin and Linial, London, and Rabinovich conjectured that every connected graph $G$ of polynomial growth admits an injective homomorphism to $\mathsf{Grid}_{n,\infty}$ for some $n < \infty$. Moreover, they conjectured that if every ball of radius $r$ in $G$ contains at most $(r+1)^\rho$ vertices, then one can take $n = O(\rho)$. The first part of this conjecture was proved by Krauthgamer and Lee in 2007. However, the second part of the conjecture is false, as Krauthgamer and Lee showed that the best possible upper bound on $n$ is $O(\rho \log \rho)$. In this paper we strengthen and extend this result in a number of ways:

* We prove an asymptotic version of the Krauthgamer--Lee theorem, which gives an asymptotically injective contraction mapping from a graph $G$ of polynomial growth to the grid graph  $\mathsf{Grid}_{n, \infty}$ with $n = O(\rho)$, where $\rho$ is the asymptotic polynomial growth rate of $G$. This confirms the stronger form of the Levin--Linial--London--Rabinovich conjecture "in the asymptotic sense."
            
* We establish a more precise relationship between the graph metrics on $G$ and on the grid to which $G$ is mapped. In particular, the mappings we construct are coarse embeddings in the sense of Gromov. This gives an affirmative answer to a question of Papasoglu.
            
* We extend the Krauthgamer--Lee theorem and all our results to the realm of Borel graphs and prove that graphs generated by free Borel actions of $\mathbb{Z}^n$ are, in an appropriate sense, universal for the class of Borel graphs of polynomial growth.

Along the way we find an alternative proof of the result of Papasoglu that graphs of polynomial growth rate $\rho < \infty$ have asymptotic dimension at most $\rho$. Furthermore, our proof works in the Borel setting and shows that Borel graphs of polynomial growth rate $\rho < \infty$ have Borel asymptotic dimension at most $\rho$, and hence they are hyperfinite. This generalizes a result of Jackson, Kechris, and Louveau (2002) from Schreier graphs of Borel group actions to arbitrary Borel graphs of polynomial growth and answers a question of Marks.

==> preliminaries.tex <==
\section{Preliminaries}
%cocycle and dynamic system
\begin{defn}[Cocycle]
Let $E$ be an equivalence relation on $X$, $\Gamma$ be an Abelian group. 
A $\Gamma$-\emphdef{cocycle} is a function $\updelta : E \to \Gamma$ such that:
\begin{itemize}
    \item $\updelta (x, x) = 0$, and 
    \item $\updelta (x, y) + \updelta (y, z) = \updelta (x, z)$. 
\end{itemize}
\end{defn}

Let $X$ be a Polish space and $E$ be an equivalence relation on $X$. 
A \emphdef{transversal} for $E$ is a set $S \subseteq X$ such that $S$ has exactly one element in every class of $E$. 
We say a Borel equivalence relation $E$ on $X$ is \emphdef{smooth} if there is a Borel transversal for $E$.
Let $\Gamma$ be an abelian group. We say a cocycle $\updelta : E \to \Gamma$ is \emphdef{smooth} if $E_\updelta \defeq \set{(x,y) \in E: \updelta(x,y) = 0}$ is smooth. 
Let $Y$ be a Polish space and $F$ be an equivalence relation on $Y$.
A \emphdef{Borel reduction} from $E$ to $F$ is a Borel map $f: X \to Y$ such that for all $x, x' \in X$ we have
$xEx' \iff f(x)Ff(x')$. 

Let $\G$ be an Abelian group.
The shift action $\alpha: \G \acts X^{\G}$ be is given by 
\[(\gamma \cdot x)(\delta) \defeq x(\delta + \gamma), \text{for all }\gamma, \delta \in \G \text{and } x \in X^{\G}. \]

We denote by $E_{\Gamma}$ the \emphdef{orbit equivalence relation}: $xE_{\Gamma}y \iff [x] = [y]$, where $[x]$ denote the orbit $\Gamma x$ of $x \in X^{\G}$. 
We denote the set of all injective functions $\Gamma \to X$ by $\mathsf{Inj}(X^{\G})$.
If $f \colon X \to \mathsf{Inj}(X^{\G})$ is a Borel reduction from $E$ to $E_{\G}$, 
define $\updelta f(x, x')$ to be the unique $\gamma \in \G$ such that $\gamma \cdot f(x) = f(x')$. 
 
\begin{theo}\label{thm:cocycle-embedding}
    Let $\G$ be a countable Abelian group. Let $E$ be a countable Borel equivalence relation on a Polish space $X$ and suppose that $\updelta \colon E \to \G$ is a smooth Borel cocycle. Then there exists 
    %a free Borel action $\alpha \colon \G \acts Y$ on some Polish space $Y$ and
    a Borel reduction $f \colon X \to \mathsf{Inj}([0, 1]^\G)$ from $E$ to $E_\G$ such that $\updelta = \updelta f$. %$G$ be a locally countable Borel graph and let $f \colon E_G \to \G$ be a Borel cocycle such that for all $x \in V(G)$, \ldots. Then there exists a free Borel action $\G \acts X$ on a Polish space $X$ and a Borel injection $V(G) \to X$ such that $f(x,y) $
\end{theo}

\begin{proof}
%Given $\gamma \in \Z^n$ and $x \in V$, define $\gamma \cdot x = y$ if there exists $y \in V$ such that $f(x, y) = \gamma$. 
    %First, we argue that it is enough to consider the case when the equivalence relation $E_\updelta$ is trivial, i.e., $\updelta(x,x') = 0$ if and only if $x = x'$.
    Since $E_\updelta$ is smooth, the quotient space $X' \defeq X/E_\updelta$ is standard Borel \todo{cite}. For $x \in X$, let $[x] \in X'$ denote the $E_\updelta$-class of $x$. Define an equivalence relation $E'$ on $X'$ by $[x] \, E'\, [x'] \,\vcentcolon \Longleftrightarrow \, x \, E \, x'$, and let $\updelta' \colon E' \to \Gamma$ be the cocycle given by $\updelta'([x], [y]) \defeq \updelta(x,y)$. Then $E_{\updelta'}$ is trivial, and since the quotient map $X \to X'$ is a Borel reduction from $E$ to $E'$, we may replace $X$, $E$, and $\updelta$ by $X'$, $E'$, and $\updelta'$ and assume, without loss of generality, that $E_\updelta$ is trivial, i.e., $\updelta(x,x') = 0$ if and only if $x = x'$. 
    
    Now we define an equivalence relation $F$ on $\G \times X$ by making $(\gamma, x)$ equivalent to $(\gamma', x')$ if and only if $x \, E \, x'$ and $\gamma - \gamma' = \updelta (x, x')$. (This is indeed an equivalence relation because $\updelta$ is a cocycle.) Note that if $(\gamma, x) \,F\, (\gamma', x')$ and $\gamma = \gamma'$, then $x = x'$ as well, since $\updelta (x, x') = \gamma - \gamma' = 0$. In other words, the members of any $F$-equivalence class have distinct first coordinates. We now claim that $F$ is a smooth equivalence relation. List the elements of $\G$ in an arbitrary order as $\gamma_0$, $\gamma_1$, \ldots{} and define a preorder $\preceq$ on $\G \times X$ by:
    \[(\gamma_i, x) \preceq (\gamma_j, x') \quad \iff \quad i \le j.\]
    Note that $\preceq$ induces a well-ordering on each $F$-equivalence class. Then we define a transversal $T$ for $F$ by picking the $\preceq$-smallest element in each $F$-equivalence class. By the Luzin--Novikov theorem, $T$ is Borel. 
    Therefore, $F$ is smooth and $Y \defeq (\G \times X)/F$ is a standard Borel space. 

    Let us now define a Borel action $\alpha \colon \G \acts Y$ as follows:
    \[
        \delta \cdot [(\gamma, x)]_F \defeq [(\delta + \gamma, x)]_F.
    \]
    This is well-defined since if $(\gamma, x) \,F\, (\gamma', x')$, then $(\delta + \gamma) - (\delta + \gamma') = \gamma -\gamma' = \updelta(x, x')$, and hence $(\delta + \gamma, x) \,F\, (\delta + \gamma', x')$. Also, this action is free since $(\gamma, x) \,F\, (\delta + \gamma, x)$ implies $\delta  = \updelta(x, x) = 0$.
    
    By \todo{cite}, there is a Borel injection $\pi \colon Y \to \mathcal{C}$. Then we can define a Borel $\G$-equivariant injective function $\pi^\ast \colon Y \to \mathcal C^{\G}$ via $\pi^\ast(y)(\gamma) \defeq \pi(\gamma \cdot y)$ for all $y \in Y$ and $\gamma \in \G$. Since the action $\G \acts Y$ is free and $\pi$ is injective, we have $\pi^\ast(Y) \subseteq \mathsf{Inj}(\mathcal C^{\G})$.
    Finally, we define $f \colon X \to \mathsf{Inj}(\mathcal{C}^\G)$ by
    \[f(x) \defeq \pi^\ast([(0, x)]_F).\]
    This is a Borel reduction from $E$ to $E_\G$. Indeed, if $x \,E\, x'$, then $f(x') = \updelta(x,x') \cdot f(x)$ and hence $f(x) \,E_\G\, f(x')$ \ep{this also shows that $\updelta f = \updelta$}. Conversely, if $f(x) \,E_\G\, f(x')$, then there is a group element $\gamma \in \G$ with $f(x') = \gamma \cdot f(x)$, which implies that $(\gamma, x) \,F\, (0, x')$ and hence $x \, E\, x'$.
\end{proof}

\begin{remk}
    The converse is also true: Let $f \colon X \to \mathsf{Inj}(\mathcal{C}^\G)$ be a Borel reduction from $E$ to $E_\G$ and let $\updelta \defeq \updelta f$. Then $\updelta$ must be smooth, since $x \,E_\updelta \, x'$ if and only if $f(x) = f(x')$.
\end{remk}


Let $X$ be a standard Borel space, then we can equip it with some Polish topology. 
Let $\mathcal K(X)$ be the collection of all compact subsets of $X$ equipped with Vietoris topology, then $\mathcal K(X)$ is Polish. 
Let $[X]^{<\infty}$ be the collection of all finite subsets of $X$. Then $[X]^{<\infty}$, as a Borel subset of $\mathcal K(X)$, is a standard Borel space. 
We say a partition of $X$ is Borel if it is a Borel subset of $[X]^{<\infty}$.  

\if0
\begin{theo}[Lusin-Novikov Theorem]
Let $X, Y$ be Polish spaces and let $f: X \to Y$ be a Borel map. 
Let $A \subseteq X$ be a Borel set such that every $y \in Y$ has countably many preimages in $A$ under $f$. 
Then $f(A)$ is a Borel subset of $Y$. 
\end{theo}
\fi
\begin{theo}[Lusin-Novikov Theorem]
Let $X, Y$ be Polish spaces and let $\pi: X \times Y \to X$ be the projection on $X$. 
Let $A \subseteq X \times Y$ be a Borel set such that every $x \in X$ has countably many preimages in $X \times Y$ under $\pi$.
Then $\pi(A)$ is a Borel subset of $X$. 
\end{theo}

\begin{Lemma}
Let $\mP$ be a partition of $X$ into clusters finite and let $E$ be such an equivalent relation on $X$: 
$xEy$ iff $x$ and $y$ are in the same cluster. 
Then $\mP$ is a Borel subset of $[X]^{<\infty}$ if and only if $E$ is a Borel subset of $X^2$.  
\end{Lemma}
\begin{proof}
For necessity: $(x, y) \in E$ iff $\exists C \in \mP (x \in C \land y \in C)$. Let
\[A = \{(x, y, C): x, y \in C, C \in \mP\} \subseteq X^2 \times [X]^{<\infty}.\]
Then $A$ is Borel. 
Let $\pi$ be the projection on $X^2$. 
Since $|\pi^{-1}((x, y))| \le 1$, by Lusin-Novikov Theorem we have $E = \pi(A)$ is Borel. 

For sufficiency, $C \in \mP$ iff $C \neq \0 \land \forall x, y \in X (x, y \in C \implies (x, y) \in E) \land \forall x, y \in X (x \in C, y \notin C \implies (x, y) \notin E)$. Let
\[A = \{(C, x, y): x, y \in C, C \in \mP\} \subseteq [X]^{<\infty} \times X^2.\]
Then $A$ is Borel. 
Let $\pi$ be the projection on $[X]^{<\infty}$. 
Since $|\pi^{-1}(C)| \le |C|^2$, by Lusin-Novikov Theorem we have $E = \pi(A)$ is Borel. 
\end{proof}

\subsection{Local Lemma}
\if0
Formally, we define \emph{coloring problems}. Let $b \in \mathbb{N}^{+}$ be a positive integer. We identify $b$ with the $b$-element set $\{0,1, \ldots, b-1\}$.
\begin{itemize}
     \item A $b$-\emphdef{coloring} of a set $S$ is a function $f: S \rightarrow b$.
    \item A \emphdef{local rule} for a graph $G$ is a function $\ru$ whose domain is $V(G)$ and such that 
        \begin{itemize}
            \item For all $x \in V(G)$ we have $\ru(x) \subseteq b^{N_G(x)}$.
            \item If $N_G(x) = \0$ then $|\ru(x)| = 1$. 
        \end{itemize}
    Given $\ru$, let $\ru^c(x) \defeq b^{N_G(x)} \backslash \ru(x)$. 
    \item A \emphdef{coloring problem} is a pair $(G, \ru)$ where $G$ is a graph and $\ru$ is a local rule. 
    \item A $k$-coloring $f: X \rightarrow k$ \emphdef{satisfies} $B$ otherwise.
    \item The \emphdef{dependency graph} of $G$ is the graph $\rel(G) = (V(G), E(\rel(G)))$ such that $(x, y) \in E(\rel(G))$ if and only if $N_G(x) \cap N_G(y) \neq \0$. 
\end{itemize}
Sometimes we wish to find a Borel coloring. 
If $V(G($ is a standard Borel space, we can speak of \emphdef{Borel coloring problem}: a pair $(G, \ru)$ where $G$ is a Borel graph and $\ru$ is a Borel local rule. 

\begin{theo}[Borel Local Lemma]
\label{thm: BLL}
Let $(G, \ru)$ be a Borel coloring problem where $G$ has a uniformly subexponential growth. 
Let $\Delta$ be the maximal vertex degree in $\rel(G)$. 
If for every $x \in V(G)$ we have
\[\frac{|\ru^c(x)|}{b^{|N_G(x)|}} < \frac{1}{e \Delta},\]
Then there exists a Borel coloring $f \in b^{V(G)}$ which satisfies $\ru$.
\end{theo}
\fi


Formally, we define \emph{constraint satisfaction problems}. Let $X$ be a set and let $k \in \mathbb{N}^{+}$ be a positive integer. We identify $k$ with the $k$-element set $\{0,1, \ldots, k-1\}$.
 \begin{itemize}
     \item A $k$-\emphdef{coloring} of a set $S$ is a function $f: S \rightarrow k$.
     \item For a finite set $D \subseteq X$, an $(X, k)$-\emphdef{constraint} (or simply a \emphdef{constraint} if $X$ and $k$ are clear from the context) with \emphdef{domain} $D$ is a set $B \subseteq k^D$ of $k$-colorings of $D$. We write $\dom(B) \defeq D$.
     \item A $k$-coloring $f: X \rightarrow k$ \emphdef{violates} a constraint $B$ with domain $D$ if the restriction of $f$ to $D$ is in $B$, and \emphdef{satisfies} $B$ otherwise.
     \item A \emphdef{constraint satisfaction problem} (a \emphdef{CSP} for short) $\B$ on $X$ with range $k$, in symbols $\B: X \rightarrow^{?} k$, is a set of $(X, k)$-constraints.
     \item A \emphdef{solution} to a CSP $\B: X \rightarrow^{?} k$ is a $k$-coloring $f: X\rightarrow k$ that satisfies every constraint $B \in \B$.
 \end{itemize}
\[\P[B] = \frac{|B|}{k^{|\dom B|}} 
 \quad\text{and}\quad \p(\B) = \sup_{B \in \B} \P[B]\]
 Sometimes we wish to find a Borel solution. 
 If $X$ is a standard Borel space, then we may speak of \emphdef{Borel CSPs} $\B: X \rightarrow^{?} k$, i.e., Borel sets $\B \subseteq [[X \times k]^{< \infty}]^{<\infty}$ of $(X, k)$-constraints. 

Given a graph $G$, 
a \emphdef{local rule} on $G$ is a CSP $\B: V(G) \rightarrow^{?} k$ of the form $\B = \{B_x: x \in V(G)\}$ where $\dom (B_x) = N_G(x)$. 
Hence if $G$ is a Borel graph, we can speak of Borel local rules. 
\begin{theo}[Borel Local Lemma]
\label{thm: BLL}
Let $G$ be a Borel graph of subexponential growth. 
Fix $k \in \N^{+}$ and let $\B: V(G) \rightarrow^{?} k$ be a Borel local rule on $G$. 
If
\[e \p(\B) \Delta (G^2)\le 1\]
then $\B$ has a Borel solution $f: V(G) \to k$. 
\end{theo}

\begin{remk}
    In the proof of Theorem~\ref{thm:Borel_padded_decomposition_1}, we will need to use the Borel LLL in a somewhat more general setting then the one we have just described. 
    Namely, suppose that in addition to a local rule  $\B: V(G) \rightarrow^{?} k$, we are given a mapping $x \mapsto k_x$ that assigns to each point a range $k_x \subseteq k$. 
    Then we may seek a solution $f: V(G) \to k$ to $\B$ with the extra property $f(x) \in k_x$ for all $x \in V(G)$. 
    It then makes sense to consider colorings $f$ where each $f(x)$ is chosen uniformly at random from $k_x$, so the probability of a constraint $B_x \in \B$ should be defined by
    \[\P(B_x) \defeq \frac{|B_x|}{k_x^{N_G(x)}}. \]   
    Thankfully, there is a straightforward way to reduce this more general set-up to the one where all sets $k_x$ are equal to each other. 
    Namely, let $n$ be a positive integer that is divisible by $1, 2, \ldots, k$.
    For each nonempty subset $S \subseteq k$, 
    fix an arbitrary function $h_S: n \to S$ such that the $h_S$-preimage of every element $s \in S$ has size exactly $n/|S|$. 
    Then, instead of picking $f(x)$ uniformly at random from $k_x$, we can pick a uniformly random integer $\phi(x) \in n$ and set $f(x) \defeq h_{k_x}(\phi(x))$. 
    For every constraint $B_x \in \B$, there is a corresponding $(V(G), n)$-constraint $B'_x$ given by 
    \[B'_x \defeq \{\phi: N_G(x) \to n: \textrm{the map } x \mapsto h_{k_x}(\phi(x)) \textrm{ is in  }\B_x\}.\]
    In this way, we replace $\B$ by an ``equivalent'' local rule $\B' \defeq \{B'_x: B_x \in \B\}: V(G) \rightarrow^{?} n$. 
    Notice also that if the local rule $\B$ and the function $x \mapsto k_x$ are Borel, then the local rule $\B'$ is also Borel, and on the other hand, if $\phi: V(G) \to n$ is a Borel solution to $\B'$, then $x \mapsto h_{k_x}(\phi(x))$ is a Borel solution to $\B$. 
\end{remk}




